DreamBench++: A Human-Aligned Benchmark for Personalized Image Generation

Personalized image generation holds great promise in assisting humans in everyday work and life due to its impressive ability to creatively generate personalized content across various contexts. However, current evaluations either are automated but misalign with humans or require human evaluations that are time-consuming and expensive. In this work, we present DreamBench++, a human-aligned benchmark that advanced multimodal GPT models automate. Specifically, we systematically design the prompts to let GPT be both human-aligned and self-aligned, empowered with task reinforcement. Further, we construct a comprehensive dataset comprising diverse images and prompts. By benchmarking 7 modern generative models, we demonstrate that DreamBench++ results in significantly more human-aligned evaluation, helping boost the community with innovative findings.

==> chapters/discussions.tex <==
\section{Discussions}
Our \dreambench showed a strong diversity in data and fair alignment with human preferences, yet there are still some known limitations that we expect future work to investigate.
\begin{itemize}[leftmargin=*]
    \item \textbf{Text prompt following evaluation can be calibrated to better align with human preference.} As shown in Table~\label{tab:main_result}, there is still a gap between \gpt evaluation and human rating for text prompt following evaluation. This could be mitigated by setting coarser scoring levels to calibrate human annotation accuracy and reduce oscillation in scoring results.
    \item \textbf{The potentials of CoT prompting and ICL are yet to be explored.} Despite the prevalence of CoT and ICL, we found that these methods yielded negative effect on our evaluation setting. We provide supplementary details of our exploration in the Appendix section with the hope of building a foundation for further improvement.
\end{itemize}

==> tabs/tab_kd.tex <==
\begin{table}[t]
\caption{
\textbf{Evaluation Aspects} of Text-to-Image Models
}
\label{tab:main_result}
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{SC-I}} & \multicolumn{3}{c}{\textbf{SC-T}} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-8}
 & \textbf{GPT} & \textbf{Human} & \textbf{DINO-I} & \textbf{CLIP-I} & \textbf{GPT} & \textbf{Human} & \textbf{CLIP-T} \\
\midrule
Textual Inversion SD v1-5 & 0.495 & 0.685 & 0.437 & 0.726 & 0.500 & 0.483 & 0.302 \\
DreamBooth SD v1-5 & 0.568 & 0.647 & 0.544 & 0.753 & \textcolor{silver}{0.581} & \textcolor{bronze}{0.543} & \textcolor{silver}{0.323} \\
DreamBooth LoRA SDXL base 1.0 & 0.594 & 0.656 & \textcolor{green}{0.628}  & \textcolor{green}{0.784}  & \textcolor{gold}{0.696}   & \textcolor{gold}{0.657} & \textcolor{gold}{0.341} \\
BLIP-Diffusion SD v1-5  & 0.406 & 0.613 & \textcolor{bronze}{0.649} & \textcolor{bronze}{0.823} & 0.394 & 0.462 & 0.286 \\
Emu2 SDXL base 1.0 & 0.614 & 0.746 & 0.539    & 0.763    & \textcolor{bronze}{0.559} & \textcolor{green}{0.513}  & \textcolor{bronze}{0.310} \\
IP-Adapter-Plus ViT-H SDXL base 1.0 & 0.418 & 0.602 & \textcolor{gold}{0.834} & \textcolor{gold}{0.917}   & 0.332    & 0.433 & 0.282 \\
IP-Adapter ViT-G SDXL base 1.0 & 0.433 & 0.591 & \textcolor{silver}{0.667} & \textcolor{silver}{0.855} & \textcolor{green}{0.510} & \textcolor{silver}{0.550} & \textcolor{green}{0.309} \\
\bottomrule
\end{tabular}
}
\end{table}



==> tabs/tab_replicate.tex <==
\begin{table}[t]
\caption{
Comparison of official results and reproduction results including
DINO-I~\cite{dinov1}, CLIP-I and CLIP-T~\cite{CLIP21} results on DreamBench~\cite{DreamBooth23}.
}
\label{tab:official_reproduction}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{T2I Model}} & \multicolumn{2}{c}{\textbf{DINO-I} & \multicolumn{2}{c}{\textbf{CLIP-I} & \multicolumn{2}{c}{\textbf{CLIP-T} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
& & \textbf{Official} & \textbf{Reproduction} & \textbf{Official} & \textbf{Reproduction} &  \\
\midrule
Textual Inversion$^\ast$~\cite{TI23} & SD v1.5 & 0.569 & 0.780 & 0.255 & 0.557 & 0.753 & 0.259 \\
DreamBooth$^\ast$~\cite{DreamBooth23} & SD v1.5 & 0.688 & 0.803 & 0.305 & 0.678 & 0.786 & 0.301 \\
DreamBooth LoRA$^\ast$~\cite{DreamBooth23} & SDXL v1.0 & - & - & - & 0.646 & 0.769 & 0.325 \\
BLIP-Diffusion~\cite{BLIPDiffusion23} & SD v1.5 & 0.594 & 0.779 & 0.300 & 0.630 & 0.784 & 0.293 \\
Emu2~\cite{emu2} & SDXL v1.0 & 0.283 & 0.766 & 0.850 & 0.287 & 0.753 & 0.842 \\
IP-Adapter-Plus ViT-H~\cite{ipadapter} & SDXL v1.0 & - & - & - & 0.846 & 0.902 & 0.272  \\
IP-Adapter ViT-G~\cite{ipadapter} & SDXL v1.0 & - & - & - & 0.681 & 0.835 & 0.295 \\
\bottomrule
\end{tabular}
}
\end{table}


